Radial and Directional Posteriors for Bayesian Neural Networks

We propose a new variational family for Bayesian neural networks. We decompose the variational posterior into two components, where the radial component captures the strength of each neuron in terms of its magnitude; while the directional component captures the statistical dependencies among the weight parameters. The dependencies learned via the directional density provide better modeling performance compared to the widely-used Gaussian mean-field-type variational family. In addition, the strength of input and output neurons learned via the radial density provides a structured way to compress neural networks. Indeed, experiments show that our variational family improves predictive performance and yields compressed networks simultaneously.

==> copied.tex <==
\setlength{\tabcolsep}{2pt}
{\renewcommand{\arraystretch}{1.4}% for the vertical padding
\begin{table*}[h]
\begin{center}
\begin{threeparttable}
\begin{footnotesize}
\begin{tabular}{l|ccccc|ccccc}
\textbf{Data} 
& \textbf{VI} & \textbf{PBP} & \textbf{Dropout} & \textbf{VMG} & \textbf{RDP} & \textbf{VI} & \textbf{PBP} & \textbf{Dropout} & \textbf{VMG} & \textbf{RDP}\\
\toprule
Bost. & 4.32$\pm$0.29 & 3.01$\pm$0.18 & 2.97$\pm$0.85 & \textbf{2.70$\pm$0.13} & $\mathit{2.81 \pm 0.17}$
          & -2.90$\pm$0.07 & -2.57$\pm$0.09 & $\mathit{-2.46\pm0.25}$ & \textbf{-2.46$\pm$0.09} & -2.60$\pm$0.03\\

Conc. & 7.19$\pm$0.12 & 5.67$\pm$0.09 & $\mathit{5.23\pm0.53}$ & \textbf{4.89$\pm$0.12} & 5.43$\pm$0.10
          & -3.33$\pm$0.02 & -3.16$\pm$0.02 & -3.04$\pm$0.09 & $\mathit{-3.01\pm0.03}$ & \textbf{-2.61$\pm$0.02}\\

Ener. & 2.65$\pm$0.08 & 1.80$\pm$0.05 & 1.66$\pm$0.19 & \textbf{0.54$\pm$0.02} & $\mathit{0.76\pm0.03}$
          & -2.39$\pm$0.03 & -2.04$\pm$0.02 & -1.99$\pm$0.09 & \textbf{-1.06$\pm$0.03} & $\mathit{-1.18\pm0.03}$\\

Kin8. & 0.10$\pm$0.00 & 0.10$\pm$0.00 & 0.10$\pm$0.00 & \textbf{0.08$\pm$0.00} & $\mathit{0.09\pm0.00}
          & ~0.90$\pm$0.01 & ~0.90$\pm$0.01 & ~0.95$\pm$0.03 & ~1.10$\pm$0.01 & \textbf{~2.17$\pm$0.00}\\

Naval & 0.01$\pm$0.00 & 0.01$\pm$0.00 & 0.01$\pm$0.00 & \textbf{0.00$\pm$0.00} & \textbf{0.00$\pm$0.00}
          & ~3.37$\pm$0.12 & ~3.73$\pm$0.01 & ~3.80$\pm$0.05 & ~2.46$\pm$0.00 & ~3.05$\pm$0.01\\

Powe. & 4.33$\pm$0.04 & 4.12$\pm$0.03 & $\mathit{4.02\pm0.18}$ & 4.04$\pm$0.04 & 4.22$\pm$0.03
          & -2.89$\pm$0.01 & -2.84$\pm$0.01 & -2.80$\pm$0.15 & -2.82$\pm$0.01 & \textbf{-0.14$\pm$0.01}\\

Prot. & 4.84$\pm$0.03 & 4.73$\pm$0.01 & $\mathit{4.36\pm0.04} & \textbf{4.13$\pm$0.02} & 4.62$\pm$0.01
          & -2.99$\pm$0.01 & -2.97$\pm$0.00 & -2.89$\pm$0.01 & -2.84$\pm$0.00 & \textbf{~1.38$\pm$0.01}\\

Wine  & 0.65$\pm$0.01 & 0.64$\pm$0.01 & \textbf{0.62$\pm$0.04} & $\mathit{0.63\pm0.01}$ & $\mathit{0.63\pm0.01}$
          & -0.98$\pm$0.01 & -0.97$\pm$0.01 & -0.93$\pm$0.06 & -0.95$\pm$0.01 & \textbf{-0.45$\pm$0.00}\\

Yacht      & 6.89$\pm$0.67 & 1.02$\pm$0.05 & $\mathit{1.11\pm0.38}$ & \textbf{0.71$\pm$0.05} & 1.13$\pm$0.10
          & -3.43$\pm$0.16 & -1.63$\pm$0.02 & -1.55$\pm$0.12 & \textbf{-1.30$\pm$0.02} & -2.36$\pm$0.04\\
\midrule
\end{tabular}
\end{footnotesize}
\vspace{-1em}
\caption{Average test set RMSE (Left) and log-likelihood (Right) on UCI regression tasks. Highest values in each task with each dataset is in bold font; while the second best is in italic font. Our method (RDP) achieves the better test likelihoods (five out of nine datasets); and reasonably good RMSE values (second best most of time).} \label{tbl:exp_regression}
%\begin{tablenotes}\scriptsize
%\item[1] \cite{graves2011practical}
%\item[2] \cite{hernandez2015probabilistic}
%\item[3] \cite{gal2016dropout}
%\item[4] \cite{louizos2016structured}
%\end{tablenotes}
\end{threeparttable}
\end{center}
\vspace{-2em}
\end{table*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%compression

\begin{table}[]
    \centering
    \begin{tabular}{c|c|c|c|c|c}
        Network & Method & Pruned architecture & FLOPs & Parameters & Error\\
  	\hline
  	
        \multirow{7}{2.5cm}{LeNet-5-Caffe  20-50-800-500}&  \textbf{RDP (ours)} &\textbf{4-7-110-66}& \textbf{125K} & \textbf{20K} & \textbf{1.0\%} \\
        
        &  BC-GNJ & 8-13-88-13&  307K & 22K & 1.0\%\\
        &  BC-GHS & 5-10-76-16& 169K & \textbf{15K} & 1.0\%\\
        &  FDOO(100K) & 2-7-112-478& \textbf{119K} & 66K & 1.1\%\\
        &  FDOO(200K) & 3-8-128-499& 163K & 81K & 1.0\% \\
        
         &  GL & 3-12-192-500& 236K & 134K & 1.0\% \\
         &  GD & 7-13-208-16& 298K & 49K & 1.1\% \\
          &  SBP & 3-18-284-283& 295K & 164K & \textbf{0.9\%} \\
        
        
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}
